Learning Temporal Rules from Noisy Timeseries Data

Events across a timeline are a common data representation, seen in different temporal modalities. Individual atomic events can occur in a certain temporal ordering to compose higher level composite events. Examples of a composite event are a patient's medical symptom or a baseball player hitting a home run, caused distinct temporal orderings of patient vitals and player movements respectively. Such salient composite events are provided as labels in temporal datasets and most works optimize models to predict these composite event labels directly. We focus on uncovering the underlying atomic events and their relations that lead to the composite events within a noisy temporal data setting. We propose Neural Temporal Logic Programming (Neural TLP) which first learns implicit temporal relations between atomic events and then lifts logic rules for composite events, given only the composite events labels for supervision. This is done through efficiently searching through the combinatorial space of all temporal logic rules in an end-to-end differentiable manner. We evaluate our method on video and healthcare datasets where it outperforms the baseline methods for rule discovery.

==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
   \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Data splits for our curated datasets are described for CATER in \ref{apx:gen_data} and for MIMIC in \ref{apx:mimic}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{For medical experiments, since querying doctors are expensive, we only had 1 trial.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{apx:optim}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix \ref{apx:mimic}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections/rule_extraction.tex <==
% \subsection{Rule Induction}
% The temporal rule formulas can be constructed given the learned weights from $\mathbf{W}$. Such construction can be carried out different ways, based on the how much is known about the rules.

\paragraph{Fixed Rule Length} If the length of the number of composite events leading to a label is known, then we can take the top-$n$ most weighted composite events to generate the rule. For each label $y_f$ dimension in $\mathbf{W}_{:, y_f}$ we can sort the composite events prediction dimension in a descending fashion with respect to their relation weights, $\mathbf{a}^{y_f} \in \mathbb{R}^{\mathcal{|X|} \cdot \mathcal{|X|} \cdot |r|} = \text{sorted}(\mathbf{W}_{:, y_f})$. Recall that every element in the vector $\mathbf{a}^{y_f}_i$ corresponds to a grounded temporal predicate $r_t^i \in r$ between two events $x_u^i, x_v^i \in \mathbf{X}$, which are used to construct a rule:
% \Karan{don't use a probability, look for paper that use the conjunctive form}
\begin{equation} 
\label{eq:rule}
    f :=  \bigwedge_{i=1}^n r_t^i(x_u^i, x_v^i) \quad \text{for} \quad r_t^i, x_u^i, x_v^i \in \text{predicate}(\mathbf{a}^{y_f}_i)
    % \ ; \  P(f)=\prod_{i=1}^n \mathbf{a}^{y_f}_i
\end{equation}
% Therefore we further regularize our model $\mathcal{L}_k = \sum_{l \in L}(\mathbf{M}_{:, l} - k)$ \Karan{choose between this and the $L_1$ norm above, ideally want values [0, 1]}

% \Karan{optimize s st y = cTMr, then look at attention to choose the combination, can pose it as a pointer network where inputs are candidate rule combinations and we have to select the correct one}
% for that composite event label in a first stage and create combinations based on those

\iffalse
In this case we look at sample pairs of $\{(\mathbf{y}, \mathbf{M_R})\}_{i=1}^m$ and maximize the information gain at each step by splitting the composite events labels by these pairwise events. The tree composed of these splits compose the predicates in the rule along the each path \cite{blockeel1998top}.The leaf nodes contain the final label with a set purity hyperparameter to terminate the splits. Then the rules along each path can similarly composed through Equation \ref{eq:rule}. 
\fi
% Through this fashion we compare against deep architectures as done in action recognition while being mindful of the latent structure of the composite event rules. We show that such a framework is able to beat the deep learning baselines while providing insightful formulas.

==> tables/ablations.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c c c c c c c}
\toprule
 & & GT Atomic & & & Pred Atomic & \\
% \cline{2-7}
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Version & mAP & Rules@1 & Rules@5 & mAP & Rules@1 & Rules@5 \\
\midrule
t=301 & .862 & .940 & .946 & .699 & .647 & .906 \\
t=150 & .771 & .880 & .936 & .659 & .578 & .810\\
t=50 & .746 & .903 & .940 & 649 & .531 & .806\\
\midrule
t=301 - dropout  &  &  &  &  &  &  \\
t=301 + fixed rela  & .857 & .943 & .946 & .702 & 747 & .920 \\
t=301 + proj  & .832 & .923 & .940 & .695 & .720 & .923\\
t=301 + $L_1$  & \textbf{.880} & \textbf{.950} & \textbf{.956} & \textbf{.714} & \textbf{.777} & .\textbf{930}\\
\bottomrule

\end{tabular}
\end{center}
\caption{We ablate the different components in our model. The base model includes all the parameters for the convolution and relation prediction ($g_\theta$) as well as the rule structure parameters ($f_\phi$), optimizing only over the label cross entropy. We first test different quantization dimensions. Based off those results we test our model without relational learning by fixing the 1d convolution as well as $g_\theta$. We also test the effect of projecting the weights to $[0,1]$ and a $L_1$ loss on $\mathbf{M_\alpha}$. \Zelin{add more baselines in this table or move this to supplementary.}}
\label{tab:ablation}
\end{table}

==> tables/baselines.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c c c c c c c}
\toprule
 & & GT Atomic & & & Pred Atomic & \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Model & mAP & Hits@1 & Hits@5 & mAP & Hits@1 & Hits@5 \\
% \midrule
% MAP & - & $.181_{\pm .000}$ & $.401_{\pm .000}$ & $.411_{\pm .000}$ & $.181_{\pm .000}$ & $.299_{\pm .000}$ & $.308_{\pm .000}$ \\
% LSTM & 1.23M & $.789_{\pm .007}$ & $.008_{\pm .004}$ & $.045_{\pm .002}$ & $.691_{\pm .008}$ & $.008_{\pm .003}$ & $.043_{\pm .002}$ \\
% LSTM Attn (L) & 1.25M & $\bf{.900_{\pm .013}}$ & $.004_{\pm .001}$ & $.045_{\pm .006}$ & $\bf{.758_{\pm .008}}$ & $.007_{\pm .004}$ & $.042_{\pm .016}$ \\
% LSTM Attn (S) & 166k & $.859_{\pm .010}$ & $.003_{\pm .000}$ & $.026_{\pm .010}$ & $\bf .750_{\pm .006}$ & $.003_{\pm .001}$ & $.042_{\pm .010}$ \\
% \midrule
% \model & 177k & $.884_{\pm .000}$ & $\bf{.963_{\pm .000}}$ & $\bf{.967_{\pm .002}}$ & $0.695_{\pm .000}$ & $\bf{.849_{\pm .006}}$ & $\bf{.965_{\pm .001}}$\\
% \bottomrule
\midrule
LSTM (L) & $.78_{\pm .00}$ & $.00_{\pm .00}$ & $.04_{\pm .00}$ & $.69_{\pm .00}$ & $.00_{\pm .00}$ & $.04_{\pm .00}$ \\
LSTM Attn (L) & $\bf{.90_{\pm .01}}$ & $.00_{\pm .00}$ & $.04_{\pm .00}$ & $\bf{.75_{\pm .00}}$ & $.00_{\pm .00}$ & $.04_{\pm .01}$ \\
LSTM Attn (S) & $.85_{\pm .01}$ & $.00_{\pm .00}$ & $.02_{\pm .01}$ & $\bf .75_{\pm .00}$ & $.00_{\pm .00}$ & $.04_{\pm .01}$ \\
% Temporal MAP & - & $.18_{\pm .00}$ & $.40_{\pm .00}$ & $.41_{\pm .00}$ & $.18_{\pm .00}$ & $.29_{\pm .00}$ & $.30_{\pm .00}$ \\
Temporal MAP & $.18_{\pm .00}$ & $.31_{\pm .00}$ & $.32_{\pm .00}$ & $.18_{\pm .00}$ & $.27_{\pm .00}$ & $.28_{\pm .00}$ \\
\midrule
\model & $.88_{\pm .00}$ & $\bf{.93_{\pm .00}}$ & $\bf{.96_{\pm .00}}$ & $.69_{\pm .00}$ & $\bf{.91_{\pm .00}}$ & $\bf{.95_{\pm .00}}$\\
\bottomrule
\end{tabular}
\end{center}
\caption{Here are the experiments from the CATER dataset against Temporal MAP and attention LSTM (large and small). In one case the models are provided timelines with ground truth atomic events (GT Atomic) and in the other we inferred the atomic events (Pred Atomic).}
% \Zelin{if LSTM does not have the ability to predict rules, consider writing as '-' instead of .00, which would look strange.}
% \Karan{we do have a method to extract rules for LSTM, but we show that it doesn't work well, see Hits@5 where some rules are recovered}
\label{tab:cater_results}
\end{table}

% We present the test mAP as well as if the top 1 and 5 rules that models produced contained the ground truth rule for that label.

% \# Params
% & 1.23M
% & 1.25M
% & 166k
% & -
% & 177k

% lstm
% 0.691	0.0068556546
% 0.0086	0.003577708764
% 0.0434	0.002880972058
% 0.7898	0.007918333158
% 0.008	0.004472135955
% 0.0454	0.00250998008
% tlp
% ave	std
% 0.6954	0.0005477225575
% 0.8494	0.006426507605
% 0.9654	0.001341640786
% 0.884	0
% 0.963	0
% 0.9676	0.00219089023
% lstm attn large
% 0.7584	0.008961026727
% 0.0074	0.004335896678
% 0.04266	0.01699935293
% 0.9002	0.01308434179
% 0.0048	0.001643167673
% 0.0454	0.006426507605
% lstm attn sm
% 0.7504	0.006107372594
% 0.0036	0.001341640786
% 0.042	0.01093160555
% 0.8596	0.0100895986
% 0.003	0
% 0.0266	0.01052615789

==> tables/related_works.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c c c c c}
    \toprule
        method & inference scale & handles noise & efficient training & rule extraction \\
        \midrule
        CEP & distributed & \cmark & & \\
        HMM & local & & \cmark & \cmark \\
        Recurrent networks & local & \cmark & \cmark & \\
        Temporal logic & local & & & \cmark \\
        Prob logic & local & \cmark & & \\
        \model{} (Ours) & local & \cmark & \cmark & \cmark \\
        \bottomrule
    \end{tabular} 
    \caption{Comparison of time series inference methods.}
    \label{tab:related_works}
\end{table}

==> tables/rule_performance.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c c c c c c c c }
        \toprule
        Max Len $n$ & $\mathbf{\bar{y}}$ & Model & Variable & Len 1 & Len 2 & Len 3 & Len 4 \\
        \midrule
        \multirow{2}*{1} & \multirow{2}*{1.0} & TLP & $\bf{1.0_{\pm .00}}$ & $\bf{1.0_{\pm .00}}$ & - & - & - \\
        & & MAP & $\bf{1.0_{\pm .00}}$ & $\bf{1.0_{\pm .00}}$ & - & - & - \\
        \midrule
        \multirow{2}*{2} & \multirow{2}*{4.0} & TLP & $\bf{.66_{\pm .02}}$ & $\bf{.96_{\pm .00}}$ & $\bf{.37_{\pm .04}}$ & - & - \\
        & & MAP & $.45_{\pm .00}$ & $.90_{\pm .00}$ & $.00_{\pm .01}$ & - & - \\
        \midrule
        \multirow{2}*{3} & \multirow{2}*{5.3} & TLP & $.43_{\pm .02}$ & $\bf{.92_{\pm .03}}$ & $.32_{\pm .09}$ & $.06_{\pm .07}$ & - \\
        & & MAP & $\bf{.45_{\pm .02}}$ & $.53_{\pm .01}$ & $\bf{.51_{\pm .02}}$ & $\bf{.32_{\pm .07}}$ & - \\
        \midrule
        \multirow{2}*{4} & \multirow{2}*{10.0} & TLP & $.23_{\pm .02}$ & $\bf{.85_{\pm .05}}$ & $.06_{\pm .04}$ & $.02_{\pm .03}$ & $.00_{\pm .01}$ \\
        & & MAP & $\bf{.46_{\pm .03}}$ & $.42_{\pm .02}$ & $\bf{.44_{\pm .2}}$ & $\bf{.56_{\pm .03}}$ & $\bf{.44_{\pm .06}}$ \\
        \bottomrule
    \end{tabular}
    \caption{For $j=1$ samples we compare model Hits@10 performances across different rule lengths. We observe the total variable length Hits for rules of all lengths that have to be learned. We break down the combined performance into the individual performance per fixed rule length $n=$ Len i, that compose the total variable performance.}
    \label{tab:rule_perf}
\end{table}

% Max rule length n=3
% Var len accuracy: 0.438 ± 0.021
% Len 1 accuracy: 0.927 ± 0.031
% Len 2 accuracy: 0.321 ± 0.095
% Len 3 accuracy: 0.067 ± 0.073
% Max rule length n=4
% Var len accuracy: 0.238 ± 0.027
% Len 1 accuracy: 0.856 ± 0.054
% Len 2 accuracy: 0.064 ± 0.048
% Len 3 accuracy: 0.024 ± 0.032
% Len 4 accuracy: 0.008 ± 0.016

% Sampled j=1 events
% Max rule length n=1
% Var len accuracy: 1.000 ± 0.000
% Len 1 accuracy: 1.000 ± 0.000
% Max rule length n=2
% Var len accuracy: 0.454 ± 0.005
% Len 1 accuracy: 0.900 ± 0.000
% Len 2 accuracy: 0.008 ± 0.010
% Max rule length n=3
% Var len accuracy: 0.457 ± 0.027
% Len 1 accuracy: 0.533 ± 0.015
% Len 2 accuracy: 0.515 ± 0.027
% Len 3 accuracy: 0.321 ± 0.073
% Max rule length n=4
% Var len accuracy: 0.468 ± 0.030
% Len 1 accuracy: 0.424 ± 0.020
% Len 2 accuracy: 0.440 ± 0.025
% Len 3 accuracy: 0.568 ± 0.039
% Len 4 accuracy: 0.440 ± 0.067

==> tables/rule_performance_before.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c c c c c c c c }
        \toprule
        Max Len $n$ & $\mathbf{\bar{y}}$ & Model & Variable & Len 1 & Len 2 & Len 3 & Len 4 \\
        \midrule
        \multirow{2}*{1} & \multirow{2}*{1.0} & TLP & $\bf{1.0_{\pm .00}}$ & $\bf{1.0_{\pm .00}}$ & - & - & - \\
        & & MAP & $.94_{\pm .00}$ & $ .94_{\pm .00}$ & - & - & - \\
        \midrule
        \multirow{2}*{2} & \multirow{2}*{4.0} & TLP & $\bf{.66_{\pm .02}}$ & $\bf{.96_{\pm .00}}$ & $\bf{.37_{\pm .04}}$ & - & - \\
        & & MAP & $.39_{\pm .01}$ & $.79_{\pm .01}$ & $.00_{\pm .00}$ & - & - \\
        \midrule
        \multirow{2}*{3} & \multirow{2}*{5.3} & TLP & $\bf{.43_{\pm .02}}$ & $\bf{.92_{\pm .03}}$ & $\bf{.32_{\pm .09}}$ & $.06_{\pm .07}$ & - \\
        & & MAP & $.10_{\pm .00}$ & $.30_{\pm .00}$ & $.00_{\pm .00}$ & $.00_{\pm .00}$ & - \\
        \midrule
        \multirow{2}*{4} & \multirow{2}*{10.0} & TLP & $\bf{.23_{\pm .02}}$ & $\bf{.85_{\pm .05}}$ & $\bf{.06_{\pm .04}}$ & $.02_{\pm .03}$ & $.00_{\pm .01}$ \\
        & & MAP & $.15_{\pm .00}$ & $.32_{\pm .00}$ & $.28_{\pm .00}$ & $.00_{\pm .00}$ & $.00_{\pm .00}$ \\
        \bottomrule
    \end{tabular}
    \caption{For $j=1$ samples we compare model Hits@10 performances across different rule lengths. We observe the total variable length Hits for rules of all lengths that have to be learned. We break down the combined performance into the individual performance per fixed rule length $n=$ Len i, that compose the total variable performance.}
    \label{tab:rule_perf}
\end{table}

% Sampled j=1 events
% Max rule length n=1
% Var len accuracy: 0.940 ± 0.000
% Len 1 accuracy: 0.940 ± 0.000
% Max rule length n=2
% Var len accuracy: 0.396 ± 0.005
% Len 1 accuracy: 0.792 ± 0.010
% Len 2 accuracy: 0.000 ± 0.000
% Max rule length n=3
% Var len accuracy: 0.101 ± 0.000
% Len 1 accuracy: 0.303 ± 0.000
% Len 2 accuracy: 0.000 ± 0.000
% Len 3 accuracy: 0.000 ± 0.000
% Max rule length n=4
% Var len accuracy: 0.150 ± 0.000
% Len 1 accuracy: 0.320 ± 0.000
% Len 2 accuracy: 0.280 ± 0.000
% Len 3 accuracy: 0.000 ± 0.000
% Len 4 accuracy: 0.000 ± 0.000

==> tables/rule_performance_thresh.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c c c c c c c c }
        \toprule
        Max Len $n$ & $\mathbf{\bar{y}}$ & Model & Variable & Len 1 & Len 2 & Len 3 & Len 4 \\
        \midrule
        \multirow{2}*{1} & \multirow{2}*{1.0} & TLP & $\bf{1.0_{\pm .00}}$ & $\bf{1.0_{\pm .00}}$ & - & - & - \\
        & & MAP & $.94_{\pm .00}$ & $ .94_{\pm .00}$ & - & - & - \\
        \midrule
        \multirow{2}*{2} & \multirow{2}*{4.0} & TLP & $\bf{.66_{\pm .02}}$ & $\bf{.96_{\pm .00}}$ & $\bf{.37_{\pm .04}}$ & - & - \\
        & & MAP & $.49_{\pm .11}$ & $.56_{\pm .26}$ & $.41_{\pm .21}$ & - & - \\
        \midrule
        \multirow{2}*{3} & \multirow{2}*{5.3} & TLP & $\bf{.43_{\pm .02}}$ & $\bf{.92_{\pm .03}}$ & $\bf{.32_{\pm .09}}$ & $.06_{\pm .07}$ & - \\
        & & MAP & $.10_{\pm .00}$ & $.30_{\pm .00}$ & $.01_{\pm .02}$ & $.00_{\pm .00}$ & - \\
        \midrule
        \multirow{2}*{4} & \multirow{2}*{10.0} & TLP & $\bf{.23_{\pm .02}}$ & $\bf{.85_{\pm .05}}$ & $\bf{.06_{\pm .04}}$ & $.02_{\pm .03}$ & $.00_{\pm .01}$ \\
        & & MAP & $.07_{\pm .04}$ & $.10_{\pm .10}$ & $.19_{\pm .10}$ & $.00_{\pm .00}$ & $.00_{\pm .00}$ \\
        \bottomrule
    \end{tabular}
    \caption{For $j=1$ samples we compare model Hits@10 performances across different rule lengths. We observe the total variable length Hits for rules of all lengths that have to be learned. We break down the combined performance into the individual performance per fixed rule length $n=$ Len i, that compose the total variable performance.}
    \label{tab:rule_perf}
\end{table}

% Sampled j=1 events
% Max rule length n=1
% Var len accuracy: 0.940 ± 0.000
% Len 1 accuracy: 0.940 ± 0.000
% Max rule length n=2
% Var len accuracy: 0.490 ± 0.113
% Len 1 accuracy: 0.564 ± 0.261
% Len 2 accuracy: 0.416 ± 0.214
% Max rule length n=3
% Var len accuracy: 0.107 ± 0.008
% Len 1 accuracy: 0.303 ± 0.000
% Len 2 accuracy: 0.018 ± 0.024
% Len 3 accuracy: 0.000 ± 0.000
% Max rule length n=4
% Var len accuracy: 0.074 ± 0.047
% Len 1 accuracy: 0.104 ± 0.109
% Len 2 accuracy: 0.192 ± 0.109
% Len 3 accuracy: 0.000 ± 0.000
% Len 4 accuracy: 0.000 ± 0.000

==> tables/video_baselines.tex <==
\begin{table}
\begin{center}
\begin{tabular}{c c c}
\toprule
Model & Inputs & Composite Event mAP\\
% \cline{2-7}
\midrule
I3D/R3D & ResNet Features + Optical Flow & .44 \\
TSN & RGB Difference + Optical Flow & .64 \\
TSM & ResNet Features & .73 \\
\midrule
Attention LSTM & Inferred Atomic Events & \bf{.75} \\
\model{} & Inferred Atomic Events & .69 \\
\bottomrule

\end{tabular}
\end{center}
\caption{We compare \model{} and our temporal baselines against video baselines on CATER}
\label{tab:video}
\end{table}
